Diffs Are Cheap, Show Me the Trajectory: An Empirical Study of Trajectory-Informed Code Review

Code review typically starts from the final diff. However, the diff reveals little about how the code was developed. Coding-agent trajectories preserve intermediate decisions, failed attempts, and validation evidence that may assist code review. We systematically investigate whether and how these trajectories can help independent review agents identify problems in the resulting code, beyond inspecting the final diff and repository. We develop a procedure that generates review comments by comparing the initial and merged versions of pull requests, and assess it against withheld human review comments. Using held-out reference implementations as comparison targets for agent-produced code, we construct a dataset linking 339 implementations of 113 DeepSWE tasks with their trajectories and 882 synthetic reference review comments. Across three coding-agent configurations and two review harnesses, we compare diff-only review, full-trajectory access, and four alternative ways of presenting and using trajectories. Full-trajectory access raises mean reference recall from 23.03% to 25.87%, but improves recall in only four of six configurations. All four alternatives improve mean reference recall over diff-only by between 4.05 and 7.32 percentage points. The gains also extend to review comments that explain task-verifier failures. Higher recall can require more tokens and longer review time, while simpler trajectory views remain competitive. These results support development trajectories as an additional source of code-review context and show that their benefits and resource costs depend on how they are presented and used.

==> authors.tex <==
% !TEX root = main.tex
% This draft intentionally omits affiliation countries.
\makeatletter
\patchcmd{\@ACM@checkaffil}
  {\ClassError{\@classname}{No country present for an affiliation}{ACM
    requires each author to indicate their country using country macro.}}
  {\ClassWarningNoLine{\@classname}{No country supplied for an affiliation}}
  {}
  {\ClassError{manuscript}{Cannot make affiliation countries optional}{The acmart affiliation check has changed.}}
% The journal layout otherwise displays emails only in the contact footnote.
\patchcmd{\@mkauthors@i}
  {\noindent\addresses}
  {\noindent
    \def\email##1##2{%
      \g@addto@macro\@currentaffiliations{%
        \unskip, \href{mailto:##2}{\nolinkurl{##2}}}}%
    \addresses}
  {}
  {\ClassError{manuscript}{Cannot display author emails}{The acmart author layout has changed.}}
\makeatother

\authorsaddresses{}

\author{Zijian Luo}
\authornote{This work was done during an internship at Microsoft.}
\affiliation{%
  \institution{Monash University}
}
\email{jack.luo@monash.edu}

\author{Pengfei Gao}
\authornote{Corresponding authors.}
\affiliation{%
  \institution{Microsoft}
}
\email{gaopengfei@microsoft.com}

\author{Dayi Lin}
\authornotemark[2]
\affiliation{%
  \institution{Microsoft}
}
\email{dayi.lin@microsoft.com}

\author{Zhiyu Fan}
\affiliation{%
  \institution{Microsoft}
}
\email{fanzhiyu@microsoft.com}

\author{Yongqiang Tian}
\affiliation{%
  \institution{Monash University}
}
\email{yongqiang.tian@monash.edu}

\author{Alejandro Carderera de Diego}
\affiliation{%
  \institution{GitHub}
}
\email{alejandro-carderera@github.com}

\author{Judge Hiciano}
\affiliation{%
  \institution{GitHub}
}
\email{judggernaut@github.com}

\author{Gemma Garriga}
\affiliation{%
  \institution{GitHub}
}
\email{gcgarriga@github.com}

\author{Qingwei Lin}
\affiliation{%
  \institution{Microsoft}
}
\email{qlin@microsoft.com}

\author{Dongmei Zhang}
\affiliation{%
  \institution{Microsoft}
}
\email{dongmeiz@microsoft.com}

\renewcommand{\shortauthors}{Luo et al.}

